TransRegex: Multi-modal Regular Expression Synthesis by Generate-and-Repair

Since regular expressions (abbrev. regexes) are difficult to understand and compose, automatically generating regexes has been an important research problem. This paper introduces TransRegex, for automatically constructing regexes from both natural language descriptions and examples. To the best of our knowledge, TransRegex is the first to treat the NLP-and-example-based regex synthesis problem as the problem of NLP-based synthesis with regex repair. For this purpose, we present novel algorithms for both NLP-based synthesis and regex repair. We evaluate TransRegex with ten relevant state-of-the-art tools on three publicly available datasets. The evaluation results demonstrate that the accuracy of our TransRegex is 17.4%, 35.8% and 38.9% higher than that of NLP-based approaches on the three datasets, respectively. Furthermore, TransRegex can achieve higher accuracy than the state-of-the-art multi-modal techniques with 10% to 30% higher accuracy on all three datasets. The evaluation results also indicate TransRegex utilizing natural language and examples in a more effective way.

==> 3-preliminaries.tex <==
%\section{Preliminaries}
\section{Background}\label{sec2}
%\subsection{Preliminaries}
Let $\Sigma$ be a finite alphabet of symbols. The set of all words over $\Sigma$ is denoted by $\Sigma^*$. The empty word and the empty set are denoted by $\varepsilon$ and $\varnothing$,  respectively.

%\begin{definition}
\textbf{Regular Expression (Regex).}
\chm{Expressions of $\varepsilon$, $\varnothing$, and $a \in \Sigma$ are regular expressions; a regular expression is also formed using the operators
$$[C] \quad r_1 | r_2\quad  r_1r_2 \quad r_1\&r_2 \quad  (r) \quad {\footnotesize \sim} r_1 \quad r_1\{m,n\}$$
where $C \subseteq \Sigma,~C\neq \{\varepsilon\}$ or $\varnothing$ is a set of characters, $m\in\mathbb{N}$, $n\in\mathbb{N}\cup\{{\infty\}}$, and $m\leq n$.}
Besides, $r?$, $r^*$, $r^+$ and $r\{i\}$ where $i\in\mathbb{N}$ are abbreviations of $r\{0,1\}$, $r\{0,\infty\}$, $r\{1,\infty\}$ and $r\{i,i\}$, respectively. $r\{m,\infty\}$ is often simplified as $r\{m,\}$.
%\end{definition}
The {\it language} $L(r)$ of a regular expression $r$ is defined inductively as follows:
$$
\begin{array}{rl}
L(\varnothing)&=\varnothing\\
L(\varepsilon)&=\{\varepsilon\}\\
L(a)&=\{a\}\\
L([C])&=C\\
L(r_1|r_2)&=L(r_1)\cup L(r_2)\\
L(r_1 r_2)&= \{vw~|~v\in L(r_1), w\in L(r_2)\}\\
%L(r_1\&r_2)&=L(r_1)\cap L(r_2)\\
L(r_1\&r_2)&= \{v~|~v\in L(r_1)\wedge v\in L(r_2)\}\\
L({\footnotesize \sim} r_1)&= \{v~|~v\notin L(r_1)\}\\
L(r\{m,n\})&=\bigcup_{m\leqslant i \leqslant n} L(r)^{i}\\
%L(r_1^*)&=\{v_1\ldots v_n ~|~ v_1,\ldots, v_n \in L(r_1), n \geq 0\}\\
\end{array}
$$

If \chm{an} expression follows the syntax above, then \chm{it} is a\emph{ valid} \chm{one}, otherwise it is \emph{ invalid}. For instance, the expression \verb|ab{1,3}| is valid, but the expression \verb|ab{1,,,,3}| is invalid.

% Given a regex $r$, its depth $d(r)$ is defined recursively as follows:
% % \begin{itemize}
% %     \item $0$ for $\varnothing, \varepsilon, a$ and $ [C]$;
% %     \item $max(d(r_1), d(r_2))$ for $r_1r_2$,  $r_1|r_2$ and $r_1\&r_2$;
% %     %\item $max(d(r_1), d(r_2))+1$ for $r_1|r_2$ and $r_1\&r_2$;
% %     \item $d(r_1)+1$ for ${\footnotesize \sim} r_1$ and $r_1\{m,n\}$.
% % \end{itemize}
% $$
% d(r) =\left \{
% \begin{array}{ll}
% 0 &\textrm{if } r = \varepsilon, \varnothing,  a \in \Sigma, \textrm{ or } [C]\\
% d(r_1) + 1 &\textrm{if } r = {\footnotesize \sim} r_1 \textrm{ or }  r_1\{m,n\} \\
% max(d(r_1), d(r_2)) &\textrm{if } r = r_1r_2, r_1 | r_2 \textrm{ or } r_1\&r_2\\
% \end{array}
% \right.
% $$
% % where $r_1, r_2$ are regexes over $\Sigma$.





\iffalse \begin{definition}
\textbf{Regular Expression (Regex).}
A regular expression over $\Sigma$ is defined inductively as follows: $\varepsilon$, $\varnothing$, $a \in \Sigma$, and $[C]$ where $C \subseteq \Sigma$ \chm{and $[$ $]$ are the character class operators} are regular expressions; for regular expressions $r_1$ and $r_2$, the disjunction $r_1 | r_2$, the concatenation $r_1r_2$, the intersection \xzw{[xzw: conjuction?]} $r_1\&r_2$, the negation ${\footnotesize \sim} r_1$, and the quantifier $r_1\{m,n\}$ where $m\in\mathbb{N}$, $n\in\mathbb{N}\cup\{{\infty\}}$, and $m\leq n$ are also regular expressions. Besides, $r?$, $r^*$, $r^+$ and $r\{i\}$ where $i\in\mathbb{N}$ are abbreviations of $r\{0,1\}$, $r\{0,\infty\}$, $r\{1,\infty\}$ and $r\{i,i\}$, respectively. $r\{m,\infty\}$ is often simplified as $r\{m,\}$.
\end{definition}
\fi



%\xzw{[xzw: May define \emph{legal}, \emph{illegal}, \emph{depth}, \emph{position} here, which are used in Section~\ref{sec:algorithm}.]}

\iffalse\begin{definition}\label{language}
The {\it language} $L(r)$ of a regular expression $r$ is defined inductively as follows:
% $L(\varnothing)=\varnothing$;
% $L(\varepsilon)=\{\varepsilon\}$;
% $L(a)=\{a\}$;
% $L([C])=C$;
% $L(r_1|r_2)=L(r_1)\cup L(r_2)$;
% $L(r_1 r_2)= \{vw~|~v\in L(r_1), w\in L(r_2)\}$;
% $L(r_1\&r_2)=L(r_1)\cap L(r_2)$;
% $L({\footnotesize \sim} r_1)= \{v~|~v\notin L(r_1)\}$;
% $L(r\{m,n\})=\bigcup_{m\leqslant i \leqslant n} L(r)^{i}$.
$$
\begin{array}{rl}
L(\varnothing)&=\varnothing\\
L(\varepsilon)&=\{\varepsilon\}\\
L(a)&=\{a\}\\
L([C])&=C\\
L(r_1|r_2)&=L(r_1)\cup L(r_2)\\
L(r_1 r_2)&= \{vw~|~v\in L(r_1), w\in L(r_2)\}\\
%L(r_1\&r_2)&=L(r_1)\cap L(r_2)\\
L(r_1\&r_2)&= \{v~|~v\in L(r_1)\wedge v\in L(r_2)\}\\
L({\footnotesize \sim} r_1)&= \{v~|~v\notin L(r_1)\}\\
L(r\{m,n\})&=\bigcup_{m\leqslant i \leqslant n} L(r)^{i}\\
%L(r_1^*)&=\{v_1\ldots v_n ~|~ v_1,\ldots, v_n \in L(r_1), n \geq 0\}\\
\end{array}
$$
\end{definition}
\fi

% \begin{definition}\label{sketch}
% \textbf{Sketch (also called template)~\cite{DBLP:journals/pacmpl/PanHXD19}.} A sketch is an expression in the grammar\xzw{[xzw: here the disjunction is the same to the meta `$|$', should use different notation]}
% \[t := [C]\,| \, t\bm{|}t \,  |\,  tt  \,| \, t\&t  \,| \, {\footnotesize \sim} t \,  |\,t\{m,n\} \,  |\, t\{\rhd,\lhd\} \,  |\, \square\]
% where $\square$ is a hole and ($\rhd,\lhd$) is a quantifier hole.
% %$\Box\blacksquare\square$
% \end{definition}
% Holes $\square$ always appear as a leaf in sketches and can be replaced with any regular expression while quantifier holes $\rhd,\lhd$ can be replaced with any two possible values for
% the $m,n$ quantifiers. 
% Each sketch implicitly represents all possible regular expressions that can be obtained by  instantiating the values of the (quantifier) holes.
% For example,  consider the sketch $t_1 =$
% \verb|h{3,}|$\square$\verb|{|$\rhd,\lhd$\verb|}[0-9]{2}[A-Z]{3,4}h{3,}| from Example~\ref{example1}, the two regular expressions \verb|h{3,}(O{1,3}){0,1}[0-9]{2}[A-Z]{3,4}h{3,}| and \verb|h{3,}J{1,3}[0-9]{2}[A-Z]{3,4}h{3,}| are actually two possible completions of the sketch $t_1$.
% %\subsection{Problem Formulation}



% \begin{definition}
% \textbf{Repair from examples.} Given  positive examples $\mathcal{P}$, negative examples $\mathcal{N}$ such that $\mathcal{P} \cap \mathcal{N} = \varnothing$, and a regular expression $r$, the {\it repair-from-examples}
% problem is to find a regular expression $r'$ that is consistent with examples --- accepts all positive
% examples (i.e., $\mathcal{P} \subseteq L(\lyt{r'})$) and rejects all negative examples (i.e., $\mathcal{N}\cap L(\lyt{r'}) = \varnothing$).
% \end{definition}
% \xzw{[xzw: be careful for (the relation of) $r$ and $r'$. The last two $r$ should be $r'$.]}\lyt{[lyt: changed]}

